Synthetic Data -- what, why and how?

This explainer document aims to provide an overview of the current state of the rapidly expanding work on synthetic data technologies, with a particular focus on privacy. The article is intended for a non-technical audience, though some formal definitions have been given to provide clarity to specialists. This article is intended to enable the reader to quickly become familiar with the notion of synthetic data, as well as understand some of the subtle intricacies that come with it. We do believe that synthetic data is a very useful tool, and our hope is that this report highlights that, while drawing attention to nuances that can easily be overlooked in its deployment.

==> Synthetic Data Survey/titlepage.tex <==
\begin{titlepage}
   \begin{center}
       \vspace*{1cm}

       \textbf{Thesis Title}

       \vspace{0.5cm}
        Thesis Subtitle
            
       \vspace{1.5cm}

       \textbf{Author Name}

       \vfill
            
       A thesis presented for the degree of\\
       Doctor of Philosophy
            
       \vspace{0.8cm}
     
       \includegraphics[width=0.4\textwidth]{university}
            
       Department Name\\
       University Name\\
       Country\\
       Date
            
   \end{center}
\end{titlepage}

==> titlepage.tex <==
\begin{titlepage}
   \begin{center}
       \vspace*{1cm}

       \textbf{Thesis Title}

       \vspace{0.5cm}
        Thesis Subtitle
            
       \vspace{1.5cm}

       \textbf{Author Name}

       \vfill
            
       A thesis presented for the degree of\\
       Doctor of Philosophy
            
       \vspace{0.8cm}
     
       \includegraphics[width=0.4\textwidth]{university}
            
       Department Name\\
       University Name\\
       Country\\
       Date
            
   \end{center}
\end{titlepage}
